X-ResQ: Reverse Annealing for Quantum MIMO Detection with Flexible Parallelism

Quantum Annealing (QA)-accelerated MIMO detection is an emerging research approach in the context of NextG wireless networks. The opportunity is to enable large MIMO systems and thus improve wireless performance. The approach aims to leverage QA to expedite the computation required for theoretically optimal but computationally-demanding Maximum Likelihood detection to overcome the limitations of the currently deployed linear detectors. This paper presents X-ResQ, a QA-based MIMO detector system featuring fine-grained quantum task parallelism that is uniquely enabled by the Reverse Annealing (RA) protocol. Unlike prior designs, X-ResQ has many desirable system properties for a parallel QA detector and has effectively improved detection performance as more qubits are assigned. In our evaluations on a state-of-the-art quantum annealer, fully parallel X-ResQ achieves near-optimal throughput (over 10 bits/s/Hz) for $4\times6$ MIMO with 16-QAM using six levels of parallelism with 240 qubits and $220~\mu$s QA compute time, achieving 2.5--5$\times$ gains compared against other tested detectors. For more comprehensive evaluations, we implement and evaluate X-ResQ in the non-quantum digital setting. This non-quantum X-ResQ demonstration showcases the potential to realize ultra-large $1024\times1024$ MIMO, significantly outperforming other MIMO detectors, including the state-of-the-art RA detector classically implemented in the same way.

==> related_work.tex <==

% % \vspace{-0.3cm}
% \section{Additional Related Work}
% \label{s:related_work}
% % \vspace{-0.1cm}
% To overcome the conventional trade-off between linear detectors (computationally-simple but suboptimal)
% and ML detectors (optimal but computationally-heavy) in MU-MIMO detection, a variety of lines of work have been studied.


% \parahead{Parallel Tree Search MIMO Detectors.}
% % \label{s:parallel_mimo}
% Non-linear detectors can enhance the detection performance at the expense of more computations~\cite{li2011multiple,yang2015fifty}. Among various non-linear detectors,  
% % \colorbox{mygreen}{\textbf{(b)}}
% parallel tree-search detectors are promising in that computation amounts can be split into multiple compute resources, reducing overall compute times.
% % aims to improve this situation, enabling near-optimal performance through parallel non-linear tree-search algorithms with massive amount of computing resources~\cite{FCSD,Wenk06,guo2006algorithm}. 
% While transistors' clock speed has stopped increasing rapidly with Moore's Law, the number of embedded transistors per chip keeps increasing nearly exponentially. With this trend, hardware that contains massive \emph{processing elements} (PEs) including GPUs and FPGAs started to be actively explored in this direction with parallel tree search algorithms~\cite{barbero2006rapid,roger2012fully,flexcore-nsdi17,nikitopoulos2018massively}. 
% % There exist various non-linear processing methods that outperform linear processing, but most of the traditional non-linear methods are operating in a sequential way and thus not suitable for parallelization, causing high compute latency~\cite{hassibi2005sphere,li2011multiple,yang2015fifty}.
% % Traditional parallel non-linear algorithms apply QR decomposition as preprocessing to transform MU-processing into tree search problems and decompose the tree into sub-problems on PEs, and the best result among sub-problem searches is filtered as a final solution. However, they cannot support flexible parallelism, so recent
% For example, Fixed-complexity Sphere Decoder (FSD)~\cite{FCSD} decomposes an ML tree search problem into multiple sub-tree search problems and then applies the \emph{greedy search} (GS) that selects the best branch per level to each of them. However, FSD cannot support flexible parallelism ($\S$\ref{s:QA_parallel_strategy}).
% % ; it can support only $
% % |\mathcal{O}|^{N_{fs}}$ levels of parallelism, where $N_{fs}$ ($0 \leq N_{fs}\leq N_t$, typically 1 or 2) is controllable user counts whose symbols are fully expanded for the decomposition.
% % To maintain the minimum processing latency and interaction overheads among PEs, a single PE is typically assigned to each path search.
% % The state-of-the art parallel algorithms~\cite{nikitopoulos2018massively,flexcore-nsdi17} transform a ML detection into an equivalent tree search problem using QR decomposition and 
% More recent parallel tree detectors such as FlexCore~\cite{flexcore-nsdi17} and MultiSphere~\cite{nikitopoulos2018massively} identify $N$ most promising paths to support any levels of parallelism, but they require additional preprocessing.

% \parahead{Physics-inspired MIMO detectors.} There are several  Physics-inspired computation methodologies apart from QA that have shown promising performance in solving the Ising problems; these methods include Coherent-Ising machines (CIM)~\cite{dopo,mcmahon2016fully,inagaki2016coherent} and Oscillator-based Ising machines~\cite{oim}. CIM can be used for calculating good-quality solutions to ML MIMO problems and provide significant performance improvements for both Large and Massive MIMO systems~\cite{rimimo,dimimo,singh2023uplink}. However, the evaluations of these methods are based only on software simulations of CIMs (with unknown anneal duration) and the performance of these methods on real hardware remains unexplored. Researchers have also explored the use of Quantum Approximate Optimization Algorithm~(QAOA), which relies on gate model-based quantum computation, for MIMO detection~\cite{cui2022general}; however, the performance evaluation of limited to either SISO systems or very small MIMO systems due to the available qubit counts.


% \vspace{-0.3cm}

